Multi-strangeness matter from ab initio calculations

Hypernuclei and hypernuclear matter connect nuclear structure in the strangeness sector with the astrophysics of neutron stars, where hyperons are expected to emerge at high densities and affect key astrophysical observables. We present the first {\em ab initio} calculations that simultaneously describe single- and double-$\Lambda$ hypernuclei from the light to medium-mass range, the equation of state for $\beta$-stable hypernuclear matter, and neutron star properties. Despite the formidable complexity of quantum Monte Carlo~(QMC) simulations with multiple baryonic degrees of freedom, by combining nuclear lattice effective field theory with a newly developed auxiliary-field QMC algorithm we achieve the first sign-problem free {\em ab initio} QMC simulations of hypernuclear systems containing an arbitrary number of neutrons, protons, and $\Lambda$ hyperons, including all relevant two- and three-body interactions. This eliminates reliance on the symmetry-energy approximation, long used to interpolate between symmetric nuclear matter and pure neutron matter. Our unified calculations reproduce hyperon separation energies, yield a neutron star maximum mass consistent with observations, predict tidal deformabilities compatible with gravitational-wave measurements, and give a trace anomaly in line with Bayesian constraints. By bridging the physics of finite hypernuclei and infinite hypernuclear matter within a single {\em ab initio} framework, this work establishes a direct microscopic link between hypernuclear structure, dense matter composition, and the astrophysical properties of neutron stars.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
